SCATTERSEARCH: Visual Querying of Scatterplot Visualizations

Scatterplots are one of the simplest and most commonly-used visualizations for understanding quantitative, multidimensional data. However, since scatterplots only depict two attributes at a time, analysts often need to manually generate and inspect large numbers of scatterplots to make sense of large datasets with many attributes. We present a visual query system for scatterplots, SCATTERSEARCH, that enables users to visually search and browse through large collections of scatterplots. Users can query for other visualizations based on a region of interest or find other scatterplots that "look similar'' to a selected one. We present two demo scenarios, provide a system overview of SCATTERSEARCH, and outline future directions.

==> graveyard.tex <==
 as our ability to capture more information and measurements improves, there is a growing need to analyze datasets with large numbers of quantitative measurements. 
